Decoupled Fitness Criteria for Reactive Systems

The correctness problem for reactive systems has been thoroughly explored and is well understood. Meanwhile, the efficiency problem for reactive systems has not received the same attention. Indeed, one correct system may be less fit than another correct system and determining this manually is challenging and often done ad hoc. We (1) propose a novel and general framework which automatically assigns comparable fitness scores to reactive systems using interpretable parameters that are decoupled from the system being evaluated, (2) state the computational problem of evaluating this fitness score and reduce this problem to a matrix analysis problem, (3) discuss symbolic and numerical methods for solving this matrix analysis problem, and (4) illustrate our approach by evaluating the fitness of nine systems across three case studies, including the Alternating Bit Protocol and Two Phase Commit.

==> new_figs/Xhat1-pr-BU.tex <==
% !TEX root = ../main.tex
\begin{align*}
    \Xhat'_1(n) &= -\frac{1}
    {5 \negc{5} \sqrt{\posc{1}}}
    \cdot
    2^{-\frac{n}{2}-3}
    \cdot e_1
    \\
    \text{where }&
    \\
    e_1 &= -4 i \left(2 \sqrt{\posc{1}}
    (-i)^n+\sqrt{2} \negc{2} \left((-i)^n-i^n\right)\right)
    \negc{1}^{n/2}
    \\
    &+4
    \left((4+i) (-i)^n+i \posc{0}
    (-i)^n+4 i^n\right) \negc{1}^{\frac{n+1}{2}}
    -e_2\cdot n - e_3
    \\
    \text{and }&
    \\
    e_2 &= -4 i
    \sqrt{10} \left((-i)^n-i^n\right) \negc{1}^{n/2}+2
    \posc{5} \left((-i)^n+i^n\right) \negc{1}^{\frac{n+1}{2}}
    \\
    &-10 \sqrt{\negc{1}} \left((-1)^n+1\right)
    \posc{1}^{n/2}+\sqrt{\negc{1}} \posc{1}^{n/
    2}
    \\
    &\left(2 \posc{0} \left((-1)^n+1\right)+5 \sqrt{2
    \posc{1}} \left((-1)^n-1\right)-\sqrt{10
    \posc{1}} \left((-1)^n-1\right)\right)
    \\
    \text{and }&
    \\
    &e_3 = 16
    \sqrt{\negc{1}} \left((-1)^n+1\right) \posc{1}^{n/
    2}+\posc{3} \sqrt{2 \negc{1}} \left((-1)^n-
    1\right) \posc{1}^{\frac{n+1}{2}}
    \\
    \text{and }&
    \\
    &\posc{a} = \sqrt{5} + a \text{ and } \negc{a} = \sqrt{5} - a
\end{align*}


==> sections/case-study-old.tex <==
% !TEX root = ../main.tex
\section{Case Studies}
\label{sec_casestudy}

We evaluate our framework on three case studies, described in detail in the subsections that follow, and summarized in Table~\ref{case-study-results}.
The symbolic method did not terminate after an hour for the larger two case studies (2PC and ABP) due to limitations imposed by the state of the art in Jordan decomposition (c.f. Section~\ref{sec_matrix_analysis}).
Therefore, Table~\ref{case-study-results} reports the results obtained by the numerical method.

In each case study we compute the fitness score for different system variants (column $M$).
Column $|M|$ represents the size (total number of states) of the system being measured, which is the product of all distributed processes.
Time refers to the total execution time, in seconds.
Column $\agg_f(M_{8192})$ refers to the $K$-approximation of the fitness score with $K=8192$, and likewise for $K=9000$.
As can be seen, the two approximations are very close within each row (identical up to at least the 3rd decimal point), which indicates convergence.
The reason we report the fitness score for K = 8192 instead of another number, say K = 8000 or K = 8500, is efficiency: 8192 the largest power of two less than 9000, and in order to compute the fitness score for K = 9000 we need to compute it anyway for K = 8192.
Our results can be reproduced using a publicly available artifact, which is structured, documented, and licensed for ease of repurposing \cite{artifactDOI}.

Let us remark that in the 2PC and ABP case studies, the systems being measured were automatically generated by a distributed protocol synthesis tool,
which is an improved version of the tool described in~\cite{ScenariosHVC2014,AlurTripakisSIGACT17}.
As our goal in this paper is fitness evaluation, we omit discussing the synthesis tool.
But, as mentioned in the introduction, evaluation of automatically synthesized systems is a promising application of our framework.

All case studies use the $\avgrate$ aggregate function.
Additionally, we use three variations of the fitness function in Fig.~\ref{fig:protocol-fitness}. This parametric fitness function suggests the possibility of constructing a library of general, reusable fitness functions. Although it was straightforward to construct fitness functions for our purposes, this library would further reduce that burden for users.

In the rest of this section we provide further details on each case study.
Some supporting figures and intermediate results are provided in
\red{Appendix~\ref{sec_cstudy-overflow}}.

\input{new_figs/case-study-results}

\subsection{Case Study \#1: Simple Communication Protocol}
This section treats the communication protocol presented in Example~\ref{ex_protocol}.
We instantiate the framework to measure the average rate at which send-ack sequences are executed and apply this instance of the framework to $M$ and $M'$ (Fig.~\ref{fig:protocol}).
The python representations of all simple communication protocol processes and fitness functions are available in \texttt{toy\_automata.py} of the artifact~\cite{artifactDOI}.


Recall that $\Sigma=\{s,t,a\}$.
Let $f_1(w) :=$ `the number of send-ack sequences of the form $st^*a$ in $w$'.
For instance (brackets $[$ and $]$ added for emphasis),
$f_1(aat [sa] [sta]a s[stta] stt[sa]) = 4$.
Additionally, let $f_2(w) := \abs{w}$ (the length of $w$) and let the fitness function $f := \angles{f_1,f_2}$. The functions $f_1,f_2$ can be represented as the DFA shown in Fig.~\ref{fig:protocol-fitness}, with $L = \{s\}$ and $R = \{a\}$.
This fitness function is measuring the number of send-ack sequences per unit of discrete time, which is analogous to the traditional measure of throughput in distributed systems.

\begin{figure}
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \input{new_figs/comm-fit1-param}
    \end{subfigure}
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        \input{new_figs/comm-fit2-param}
    \end{subfigure}
    \caption{The DFA representations of $f_1$ and $f_2$ for the case studies, parameterized by the set of labels $\Sigma$, as well as a set of {\em left endpoints} $L\subseteq\Sigma$ and {\em right endpoints} $R\subseteq\Sigma$. $\overline{L} = \Sigma\setminus L$ and likewise for $\overline{R}$.}
    \label{fig:protocol-fitness}
\end{figure}

As reported in Table~\ref{case-study-results}, the system that uses the good receiver has a fitness score of about $0.25$ and the system using the bad receiver a score of about $0.138$. These scores are {\em interpretable} in that they have units: send-ack sequences per unit of discrete time.
Hence, the framework deems the good receiver as more fit and this determination aligns with our intuitions.
Because this example is relatively small, Mathematica was able to compute the exact fitness scores of these systems. The system that uses the good receiver has a fitness score of exactly $1/4$ (obtained after 34 seconds) and the system that uses the bad receiver has a score of exactly $\frac{5-\sqrt{5}}{20}\approx 0.138$ (obtained after 563 seconds).

\subsection{Case Study \#2: Two Phase Commit (2PC)}
Two phase commit (2PC) is a protocol for making transactional changes to a distributed database atomically; if one sub-operation of the transaction is aborted at one remote database, so too must the sub-operations at all other remote databases. In our model of 2PC, a user initiates a transaction by synchronizing with a {\em transaction manager} on the label $x$. The transaction is complete when the transaction manager synchronizes with the user on label \textit{fail} or \textit{succ}. We omit the details of the intermediate exchanges between the transaction manager and database managers.

The fitness function for this case study is as depicted in Fig.~\ref{fig:protocol-fitness}, with $L = \{x\}$, $R = \{\textit{fail},\textit{succ}\}$, and $\Sigma$ has a total of 18 labels. This fitness function measures the rate at which transactions are initiated and then completed.

We study three 2PC implementations, each using a different transaction manager LTS.
The system labeled H in Table~\ref{case-study-results} uses a previously manually constructed transaction manager that the synthesis tool was also able to discover automatically, while the systems labeled A1 and A2 use new transaction managers generated by the synthesis tool.
The automatically generated transaction managers  have 12 states each and it is therefore hard to tell at a glance which will give rise to the most efficient protocol.
Our tool automatically reports, in fractions of a second, a fitness score of about $0.083$ for both systems
 H and A2, and a score of about $0.078$ for system A1.

\subsection{Case Study \#3: Alternating Bit Protocol (ABP)}
The Alternating Bit Protocol (ABP) allows reliable communication over an unreliable network. As with the prior two case studies, we use the fitness function depicted in Fig.~\ref{fig:protocol-fitness}, except with $L = \{\textit{send}\}, R = \{\textit{done}\}$, and $\Sigma$ of size 12. Similar to case study \#1 we are measuring the rate of send-done sequences.

In~\cite{AlurTripakisSIGACT17}, the authors present a method to automatically synthesize (distributed) ABP sender and receiver processes. Here, we evaluate the fitness of the ABP variants that use these various synthesized processes.
Together the synthesized sender and receiver processes have 14 states, which again makes manual determinations about the fitness very challenging -- even more so due to the distributed nature of the problem. It is no longer necessarily a question of which sender or receiver is better than the other sender or receiver, but a question of which combination of sender and receiver is best.
Once again, our framework allows to automatically make this determination in a matter of seconds.

The systems are ranked by fitness in the following order: HH, HA, AH, AA.
H stands for human-designed (and then also rediscovered during synthesis) and A stands for newly discovered during synthesis.
The first position is for the sender process and the second for the receiver.
In this case study, the newly discovered processes do worse than the manually constructed processes.
The difference in fitness scores is meaningful: HH takes an average of 59 units of time to complete each send-done sequence, while AA take about 72 units. Therefore, over the same amount of time, AA will complete 20\% fewer sequences on average. AH and HA will both complete about 9\% fewer messages than HH.

